Fixed points of K-Fibonacci sequences

A $K$-Fibonacci sequence is a binary recurrence sequence where $F_0=0$, $F_1=1$, and $F_n=K\cdot F_{n-1}+F_{n-2}$. These sequences are known to be periodic modulo every positive integer greater than $1$. If the length of one shortest period of a $K$-Fibonacci sequence modulo a positive integer is equal to the modulus, then that positive integer is called a $\textit{fixed point}$. This paper determines the fixed points of $K$-Fibonacci sequences according to the factorization of $K^2+4$ and concludes that if this process is iterated, then every modulus greater than $3$ eventually terminates at a fixed point.

==> bibliography.tex <==
\begin{thebibliography}{10}

\bibitem{Bouazzaoui}
Zakariae Bouazzaoui.
\newblock {F}ibonacci numbers and real quadratic p-rational fields.
\newblock {\em Periodica Mathematica Hungarica}, 81(1):123--133, 2020.

\bibitem{Bouazzaoui_2}
Zakariae Bouazzaoui.
\newblock On periods of {F}ibonacci sequences and real quadratic p-rational
  fields.
\newblock {\em Fibonacci Quarterly}, 58(5):103--110, 2020.

\bibitem{cerda-morales}
Gamaliel Cerda-Morales.
\newblock On generalized {F}ibonacci and {L}ucas numbers by matrix methods.
\newblock {\em Hacettepe Journal of Mathematics}, 42(2):173--179, 2013.

\bibitem{[Everest]}
G.~Everest, A.~van~der Poorten, I.~Sharplinski, and T.~Ward.
\newblock {\em Recurrence Sequences}.
\newblock Rhode Island, USA: American Mathematical Society, 2004.

\bibitem{[Falcon]}
Sergio Falcon and {\'A}ngel Plaza.
\newblock k-{F}ibonacci sequences modulo m.
\newblock {\em Chaos, Solitons \& Fractals}, 41(1):497--504, 2009.

\bibitem{[Fulton_Morris]}
John Fulton and William Morris.
\newblock On arithmetical functions related to the {F}ibonacci numbers.
\newblock {\em Acta Arithmetica}, 2(16):105--110, 1969.

\bibitem{Harrington}
Joshua Harrington and Lenny Jones.
\newblock A note on generalised {W}all--{S}un--{S}un primes.
\newblock {\em Bulletin of the Australian Mathematical Society},
  108(3):373--378, 2023.

\bibitem{Jones2023}
Lenny Jones.
\newblock Generalized {W}all-{S}un-{S}un primes and monogenic
  power-compositional trinomials.
\newblock {\em Albanian Journal of Mathematics}, 17(2), 2023.

\bibitem{Jones2024}
Lenny Jones.
\newblock A new condition for $ k $-{W}all--{S}un--{S}un primes.
\newblock {\em Taiwanese Journal of Mathematics}, 28(1):17--28, 2024.

\bibitem{[Lagrange]}
J.~L. Lagrange.
\newblock Oeuvres de {L}a{G}range.
\newblock {\em Gauthier Villars, Paris}, 7:5--182, 1877.

\bibitem{Renault}
Marc Renault.
\newblock The period, rank, and order of the (a, b)-{F}ibonacci sequence mod m.
\newblock {\em Mathematics Magazine}, 86(5):372--380, 2013.

\bibitem{[A106291]}
Neil J.~A. Sloane and The OEIS~Foundation Inc.
\newblock The on-line encyclopedia of integer sequences {A}106291.
\newblock http://oeis.org/A106291, 2021.

\bibitem{[Sun-Sun]}
Zhi-Wei Sun.
\newblock {F}ibonacci numbers and {F}ermat's last theorem.
\newblock {\em Acta Arithmetica}, 60(4):371--388, 1992.

\bibitem{[Trojovska]}
Eva Trojovsk\'a.
\newblock On periodic points of the order of appearance in the {F}ibonacci
  sequence.
\newblock {\em Mathematics}, 8(5):773, 2020.

\begingroup % no newpage
\let\cleardoublepage\relax
\bibitem{[Wall]}
Donald~Dines Wall.
\newblock {F}ibonacci series modulo m.
\newblock {\em The American Mathematical Monthly}, 67(6):525--532, 1960.
\end{thebibliography}
\endgroup


